CLUTR: Curriculum Learning via Unsupervised Task Representation Learning

Reinforcement Learning (RL) algorithms are often known for sample inefficiency and difficult generalization. Recently, Unsupervised Environment Design (UED) emerged as a new paradigm for zero-shot generalization by simultaneously learning a task distribution and agent policies on the generated tasks. This is a non-stationary process where the task distribution evolves along with agent policies; creating an instability over time. While past works demonstrated the potential of such approaches, sampling effectively from the task space remains an open challenge, bottlenecking these approaches. To this end, we introduce CLUTR: a novel unsupervised curriculum learning algorithm that decouples task representation and curriculum learning into a two-stage optimization. It first trains a recurrent variational autoencoder on randomly generated tasks to learn a latent task manifold. Next, a teacher agent creates a curriculum by maximizing a minimax REGRET-based objective on a set of latent tasks sampled from this manifold. Using the fixed-pretrained task manifold, we show that CLUTR successfully overcomes the non-stationarity problem and improves stability. Our experimental results show CLUTR outperforms PAIRED, a principled and popular UED method, in the challenging CarRacing and navigation environments: achieving 10.6X and 45\% improvement in zero-shot generalization, respectively. CLUTR also performs comparably to the non-UED state-of-the-art for CarRacing, while requiring 500X fewer environment interactions.

==> sections/checklist.tex <==

\newpage 




% For the paper checklist
\newcommand{\answerYes}[1][]{\textcolor{blue}{[Yes] #1}}
\newcommand{\answerNo}[1][]{\textcolor{orange}{[No] #1}}
\newcommand{\answerNA}[1][]{\textcolor{gray}{[N/A] #1}}
\newcommand{\answerTODO}[1][]{\textcolor{red}{\bf [TODO]}}

%%% BEGIN INSTRUCTIONS %%%
\begin{comment}
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
\end{comment}



%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We have submitted our code and instructions including training and testing scripts as a zip file with the submission. Saved checkpoints and data will also be made public upon acceptance or during the rebuttal phase. The appendix also details experimental details with hyperparameters.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> sections/intro_alternate_paragraphs.tex <==
Deep Reinforcement Learning (RL) has shown exciting progress in the past decade solving many challenging domains including Atari~\cite{atari}, Dota~\citet{dota}, Go~\citet{go}. However, deep RL algorithms are critiqued for their sample-inefficiency. Curriculum Learning (CL) algorithms have shown promising results on improving the sample efficiency of Deep RL algorithms by training the RL agents with a curriculum of increasingly difficult sequence of tasks: starting from the easy ones and then progressively increasing the difficulty (~\cite{cl0}, ~\cite{cl1}). Deep RL agents are also notorious for their brittleness, performing poorly or simply failing on tasks which differ only slightly from the tasks they were trained on (~\cite{generalization0}, ~\cite{generalization1}, ~\cite{generalization2}). A more recent class of Unsupervised CL algorithms, called Unsupervised Environment Design (UED), have shown impressive zero-shot generalization by training the agents on a diverse distribution of tasks generated from an underspecified paramater space of the environment. PAIRED (~\citet{paired}) is one of the most popular and principled UED algorithms. It trains a teacher agent using adversarial training, where the agent to be trained (also called protagonist) along with a second agent, called the antagonist, are employed and trained on the same tasks generated by the teacher agent, while the teacher itself optimizes the regret  defined as the difference of  the antagonist and the agent's return. Theoretically this regret optimization incentivizes the PAIRED teacher to generate feasible but challenging tasks for the agent and is adopted by the many contemporary UED algorithms (e.g., ~\citet{accel}, ~\citet{dcd}).


Reinforcement Learning has shown exciting progress in the past decade solving many challenging domains including Atari~\cite{atari}, Dota~\citet{dota}, Go~\citet{go}. However, RL is also notorious for sample inefficiency and a lack of generalization. Curriculum Learning (CL) algorithms have been shown to improve sample efficiency by training the agents on a sequence of tasks\footnote{To avoid confusion, throughout this paper we will use the term Environment as the Simulator and Task to refer a concrete MDP from an underspecified one---often referred as Environment in UED literature---e.g., location of obstacles for navigation}, starting from the easy ones and then progressively increasing the difficulty. CL algorithms aim to present ``just-the-right-amount-of-challenge" to the agents by generating tasks at the frontier of the agent's capabilities. A more recent class of Unsupervised CL algorithms, called Unsupervised Environment Design (UED), have shown impressive zero-shot generalization by training the agents on a diverse distribution of tasks generated from an underspecified paramater space of the environment. PAIRED (~\citet{paired}) is one of the most popular and principled UED algorithms. It trains a teacher agent using adversarial training, where the agent to be trained (also called protagonist) along with a second agent, called the antagonist, are employed and trained on the same tasks generated by the teacher agent, while the teacher itself optimizes the regret  defined as the difference of  the antagonist and the agent's return. Theoretically this regret optimization incentivizes the PAIRED teacher to generate feasible but challenging tasks for the agent and is adopted by the many contemporary UED algorithms (e.g., ~\citet{accel}, ~\citet{dcd}).

%Attempts have been made to improve it by augmenting it with other techniques such as level replay(~\cite{dcd}). 


In spite of the generalization capabilities of PAIRED, it is still sample inefficient. Training a regret-based teacher is hard and often deemed as the Achilles' heel of UED algorithms(~\cite{accel}). PAIRED formulates the teacher as an RL agent which receives a sparse reward only after generating a fixed-length sequence of environment parameters (e.g., location of the obstacles for navigation)

involves a long-horizon credit assignment in an exponential parameter space. The teacher is typically formulated as an RL agent which receives a sparse reward only after generating a fixed-length sequence of environment parameters (e.g., location of the obstacles for navigation). Additionally, the teacher agent also faces a combinatorial explosion problem due to parameter space being permutation invariant---e.g., for a navigation task the same set of obstacles can be generated by a plethora of different sequence of parameters, on the order of the factorial of the number of blocks. More importantly, the teacher needs to simultaneously learn a task manifold as well as navigate it to create an effective curriculum, which is difficult due to the task manifold evolving over time. The task manifold is an important aspect of curriculum learning algorithms enabling the teacher to find tasks at the frontier of agents' capabilities. Moreover, this task manifold is learned indirectly while optimizing for regret without any explicit regards to the actual task structures.

% Hence, CL algorithms attempt to find `just-the-right-amount-of-challenging' tasks at the frontier of the agent's capabilities.

%deep RL agents still prove to be brittle, often failing to transfer to environments only slightly different from those encountered during training [44, 9]. 

% PAIRED’s specific adversarial approach to environment design ensures a useful robustness characterization of the final student policy in the form of a minimax regret guarantee [31]—assuming that its underlying teacher-student multi-agent system arrives at a Nash equilibrium [NE, 24].  
%\footnote{To avoid confusion, throughout this paper we will use the term Environment as the Simulator and Task to refer a concrete MDP from an underspecified one---often referred as Environment in UED literature---e.g., location of obstacles for navigation}

% add motivation of CL : % slightly harder than it can already solve or, on the tasks the agent can solve them already but can obtain better returns.



%In spite of the generalization capabilities of PAIRED, it is sample inefficient. Attempts have been made to improve PAIRED by augmenting it with other techniques such as environment editing capabilities~\cite{} and level replay~\cite{}. 
%All of the current UED methods involve training the teacher agent  with a sparse-reward RL problem which requires solve a long-horizon credit assignment problem---often deemed as the Achilles' heel of UED algorithms~\cite{accell}. Also, a credit assignment over the parameter sequence, for example over the position of obstacles in the grid environments, often does not make much practical sense. Most importantly, these methods learns task structures indirectly, which we argue is one of the most important aspects of Curriculum Learning algorithms. A curriculum learning algorithm tries to progressively generate environments at the horizon of the agents' capabilities. Consider an human teacher, who present a sequence of  exercises to the student---each exercise being a bit more difficult but also similar to the previous problem(s). Hence, the capability to generate `similar' but slightly harder tasks is a core property of any CL algorithm. The existing UED algorithms learn the task structures indirectly, for example PAIRED learns it indirectly via credit assignment while optimizing for the regret objective, contributing to sample inefficiency. Additionally, the teacher algorithm faces a combinatorial explosion as they  generate the sequence of parameters, e.g., obstacle locations, as the same set of obstacles can be generated by a plethora of different sequence of numbers, in order of the factorial of the number of blocks. Finally, the existing UED methods use different model architectures for the teachers for different problems by tailoring them to suit different parameter space. 

%We present CLUTR: Curriculum Learning via Unsupervised Task Representation Learning aiming to improve efficiency and effectiveness of UED algorithms by addressing the above mentioned points. At the heart of our method is a generative model that learns a latent representation of tasks. A `good' latent task space, would portray a local neighborhood structure---similar tasks being mapped to a closed neighborood in the latent space. We build our method on top of PAIRED: the teacher agent in CLUTR samples from the latent task instead of sampling from the parameter space and the generative model is used to obtain concrete parameters of the task. In contrast to the PAIRED teacher which tries to build the tasks from scratch one parameter at a time, CLUTR teacher `selects' concrete tasks  by sampling the latent space and induces curriculum by navigating the latent space. With the introduction of this latent space, we decouple the problem of learning task structure from the problem of inducing the curriculum and avoids the combinatorial explosion problem. The latent generative model is trained in an unsupervised manner from random tasks sampled from the underspecified parameter space without requiring any costly interaction with the simulator. Practically, CLUTR teacher can also be trained with a single-step RL formulation---avoiding any long-horizon credit assignment. Finally, as the theoretical properties of PAIRED is agnostic of the teacher model, they also hold in CLUTR. 

\begin{comment}
In summary, we make the following contributions: 

\begin{itemize}
    \item We introduce CLUTR, a novel unsupervised Curriculum Learning algorithm which utilizes unsupervised latent task representation learning. Built on top of PAIRED, it holds similar Theoretical properties and guarantees.
    \item We address several practical challenges faced by current the UED teacher training methods: tangled task representation learning and curriculum induction, solving long-horizon credit assignment problem and combinatorial explosion of the paramaters
    \item Our experimental results show CLUTR outperforms PAIRED both, in terms of generalisation and sample-efficiency, in MiniGrid and CarRacing environments.

    \item CLUTR also outperforms and/or is comparable with previous SOTA UED methods while being much simpler to implement. CLUTR even outperforms the CarRacing SOTA\cite{} in 8 out of the 20 test tracks.
\end{itemize}
\end{comment}

%The latent generative model is trained in an unsupervised manner from random tasks sampled from the underspecified parameter space. This unsupervised approach allow us to avoid any interaction with the simulator, which is typically an order of magnitude expensive than random sampling.  

%“Indeed, the Achilles' heel of prior UED methods, like PAIRED, is the difficulty of training the teacher, typically entailing an RL problem with sparse rewards and long-horizon credit assignment" \cite{accel} <- add this it is more general, where ??

%the continuous single-step formulation can solve the problem of sparse rewards

%In spite of the generalization capabilities of PAIRED, we notice that i) it is highly sample inefficient. Specially,  training the environment agent is very difficult, deemed as the Achilles' heel of the UED algorithms\cite{accel} requiring to solve an RL problem with sparse rewards and long-horizon credit assignment.  ii) the environment agent generates a sequence of numbers (e.g, position of blocks) to generate the environment and hence faces a combinatorial explosion---different permutation of the same (or part of) parameter vector are translated to the same task, which it tries to learn via a sparse-reward credit assignment, and iii) PAIRED does not explicitly notion of the task structure, i.e., a very important aspect for curriculum learning algorithms as they aim to generate similar-but-slightly-more-difficult next-tasks. 

%We present Curriculum Learning via Unsupervised Task Representation Learning (CLUTR) aiming to address the above mentioned points. We propose learning a latent task representation from the underspecified task description/parameter space in an unsupervised manner to augment UED algorithms---instead of sampling from the parameter space, the environment agent now "selects" points in the latent space and in the course of training tries to generate progressively difficult environments by navigating this latent space. We formulate the environment generation as a contextual bandit problem and learn the latent task representation in an unsupervised manner from randomly generated environments. Our experiments show ... 

%we can think of pretrained vae as a strong prior on task structure whereas in paired, the task structure is learned from scratch; as a result, it is taking a long time to learn.

%VAE gives a structure but it is not adaptive. we should be careful when criticizing paired.
\begin{comment}
In summary  we have the following contributions:

i) We show, to the best of the authors' knowledge, how UED algorithms can be augmented with latent task representations learned in an unsupervised manner without any costly interaction with the environment.

ii) Our experimental results show, CLUTR outperforms PAIRED in terms of both generalisation and sample-efficiency.

iii) CLUTR shows better and/or comparable performance to other methods that augment UEDs with Level-Editing capabilities / PLR, while being much simpler to implement.  

\end{comment}
